Optimizing the ecological connectivity of landscapes with generalized flow models and preprocessing

In this paper we consider the problem of optimizing the ecological connectivity of a landscape under a budget constraint by improving habitat areas and ecological corridors between them. We consider a formulation of this problem in terms of graphs in which vertices represent the habitat areas and arcs represent a probability of connection between two areas that depend on the quality of the respective corridor. We propose a new generalized flow model that improves existing models for this problem and an efficient preprocessing algorithm that reduces the size of the graphs on which generalized flows is computed. Reported numerical experiments highlight the benefice of these two contributions on computation times and show that larger problems can be solved using them. Our experiments also show that several variants of greedy algorithms perform relatively well on practical instances while they return arbitrary bad solutions in the worst case.

==> custom.tex <==
% problem environment
\usepackage{mdframed, tabularx,lipsum,environ,amsmath,amssymb,hyperref}
\makeatletter
\newcommand{\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand{\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand{\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question
\NewEnviron{problem}{
  \problemtitle{}\probleminput{}\problemquestion{}% Default input is empty
  \BODY% Parse input
  \par\addvspace{0\baselineskip}
  \noindent
  \begin{mdframed}
    \begin{tabularx}{\textwidth}{l X c}
      \multicolumn{2}{l}{\large \textsc{\@problemtitle}} \\% Title
      \textbf{Input:} & \@probleminput \\% Input
      \textbf{Question:} & \@problemquestion% Question
    \end{tabularx}
  \end{mdframed}
  \par\addvspace{.5\baselineskip}
}
\makeatother

% optimisation problem environment
\makeatletter
\newcounter{optimisation_program}
\newcounter{constraint}
\newcommand{\name}[1]{\gdef\@name{\def\tmp{#1}\ifx\tmp\empty\Alph{optimisation_program}\else\tmp\fi}}% problem name
\newcommand{\sense}[1]{\gdef\@sense{#1}}% problem sense
\newcommand{\objective}[1]{\gdef\@objective{#1}}% problem objective
\newcommand{\constraints}[1]{\gdef\@constraints{#1}}% problem constraints
\newcommand{\constraint}[2]{& #1 & #2 & \refstepcounter{constraint} (\Alph{optimisation_program}\theconstraint)\\}% problem constraint
\NewEnviron{optimisation_program}{
  \name{}\sense{min}\objective{}\constraints{}% Default input is empty
  \stepcounter{optimisation_program}% step optimisation_program number
  \setcounter{constraint}{0}% init constraints number
  \BODY% parse commands
  \def\arraystretch{1.30}    
  
  \begin{table*}[!ht]
    \centering
    $\textnormal{\@name}\left\{\begin{tabular}{rlll}
    \textnormal{\@sense}& \@objective &\\
    \textnormal{s.t.}\@constraints
    \end{tabular}\right.$
  \end{table*} 
}
\makeatother



% Proof environments
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{claim}{Claim}
\newtheorem{corollary}{Corollary}
\newtheorem*{definition}{Def}


\newcommand{\Implies}[2]{\noindent$\text{\ref{#1}}\implies\text{\ref{#2}}$: }% X => Y



% case list
\newenvironment{caseof}{}{\vskip.5\baselineskip}
\newcommand{\case}[3]{\vskip.5\baselineskip\par\noindent {\bfseries \label{#2}#1:} #3}
